Offline Training of Language Model Agents with Functions as Learnable Weights

Researchers and practitioners have recently reframed powerful Large Language Models (LLMs) as agents, enabling them to automate complex tasks largely via the use of specialized functions. To facilitate the development of LLM agents, we present a novel paradigm of training LLM agents without modifying the LLM weights, which is particularly useful when the LLMs are difficult or inaccessible for modifications. Inspired by how humans continuously forge tools to adapt to real-world tasks, rather than change our biological structure to fit a static set of tools, we propose to progressively forge agent's functions to better solve the downstream tasks instead of modifying the LLM weights. By treating the functions as learnable `agent parameters' and leveraging the fundamental idea of model training in artificial intelligence, we develop AgentOptimizer that employs the LLM to update agents' functions and devise an agent training algorithm with two strategies, roll-back, and early-stop, to streamline the training process. With extensive experiments, we showcase that the agent training paradigm could significantly improve the performance of representative LLM agents in various downstream tasks. We also study the behavior of the agent training regarding aspects like the learning curve and domain transferability.

==> macro-math.tex <==
% %================================ PREAMBLE ==================================
% \allowdisplaybreaks

% %---------- Spacing ------------
% \setlength{\parindent}{0pt}
% \setlength{\parskip}{9pt}

% % --------- Begin Preamble -------------
% \newcommand{\E}{{\mathbb E}}
% \newcommand{\N}{{\mathbb N}}
% \newcommand{\R}{{\mathbb R}}
% \newcommand{\U}{{\mathbb U}}
% \newcommand{\I}{{\mathbf I}}
% \newcommand{\bx}{{\mathbf{x}}}
% \renewcommand{\P}{{\textbf P}}
% \newcommand{\bP}{{\mathbb P}}
% \newcommand{\bE}{{\mathbb E}}
% \newcommand{\K}{{\textbf K}}
% \newcommand{\A}{{\textbf A}}
% \newcommand{\bB}{{\textbf B}}
% \newcommand{\bS}{{\mathbf{S}}}
% \newcommand{\bV}{{\textbf V}}
% \newcommand{\bU}{{\textbf U}}
% \newcommand{\bX}{{\textbf X}}
% \newcommand{\bY}{{\textbf Y}}
% \newcommand{\bZ}{{\textbf Z}}
% \renewcommand{\d}{{\textbf d}}
% \newcommand{\cA}{{\mathcal A}}
% \newcommand{\cC}{{\mathcal C}}
% \newcommand{\cH}{{\mathcal H}}
% \newcommand{\cD}{{\mathcal D}}
% \newcommand{\cF}{{\mathcal F}}
% \newcommand{\cN}{{\mathcal N}}
% \newcommand{\cX}{{\mathcal X}}
% \newcommand{\cY}{{\mathcal Y}}
% \newcommand{\cW}{{\mathcal W}}
% \newcommand{\cB}{{\mathcal B}}
% \newcommand{\cS}{{\mathcal S}}
% \newcommand{\cR}{{\mathcal R}}
% \newcommand{\cP}{{\mathcal P}}
% \newcommand{\cQ}{{\mathcal Q}}
% \newcommand{\cI}{{\mathcal I}}
% \newcommand{\nabf}{{\nabla f}}
% \newcommand{\hs}{{\hat s}}
% \newcommand{\hh}{{\hat h}}
% \newcommand{\hg}{{\hat g}}
% \renewcommand{\v}{{\mathbf v}}
% \renewcommand{\u}{{\mathbf u}}
% \newcommand{\w}{{\mathbf w}}
% \newcommand{\tw}{{\tilde \w}}
% \newcommand{\tf}{{\tilde f}}
% \newcommand{\tx}{{\tilde \x}}
% \newcommand{\tg}{{\tilde g}}
% \newcommand{\tO}{{\tilde O}}
% \newcommand{\hw}{{\hat \w}}
% \newcommand{\bg}{{\bar g}}
% \newcommand{\bw}{{\bar \w}}
% \newcommand{\h}{{\mathbf h}}
% \newcommand{\g}{{\mathbf g}}
% \newcommand{\x}{{\mathbf x}}
% \newcommand{\rb}{{\mathbf r}}
% \newcommand{\hx}{{\hat \x}}
% \newcommand{\y}{{\mathbf y}}
% \newcommand{\z}{{\mathbf z}}
% \newcommand{\p}{{\mathbf p}}
% \newcommand{\q}{{\mathbf q}}
% \newcommand{\e}{{\mathbf e}}
% \renewcommand{\b}{{\mathbf b}}
% \renewcommand{\a}{{\mathbf a}}
% \newcommand{\n}{{\mathbf n}}
% \newcommand{\bTheta}{{\boldsymbol \Theta}}
% \newcommand{\bdelta}{{\boldsymbol \delta}}
% \newcommand{\bDelta}{{\boldsymbol \Delta}}
% \newcommand{\btheta}{{\boldsymbol \theta}}
% \newcommand{\ttheta}{{\tilde \btheta}}
% \newcommand{\htheta}{{\hat \btheta}}
% \newcommand{\bSigma}{{\boldsymbol \Sigma}}
% \newcommand{\bnu}{{\boldsymbol \nu}}
% \newcommand{\bmu}{{\boldsymbol \mu}}
% \newcommand{\1}{{\boldsymbol 1}}
% \newcommand{\0}{{\boldsymbol 0}}
% \newcommand{\red}[1]{\textcolor{red}{AS: #1}}
% \newcommand{\blue}[1]{\textcolor{blue}{#1}}
% \newcommand{\conf}{{\texttt{conf}}}
% \newcommand{\train}{\text{train}\xspace}
% \newcommand{\test}{{\text{test}}\xspace}
% \newcommand{\val}{{\text{val}}\xspace}
% \newcommand{\Loss}{{\texttt{Loss}}}
% \newcommand{\worst}{\text{worst}\xspace}
% \newcommand{\avg}{\text{avg}\xspace}
% \newcommand{\LexiMin}{\text{LexiMin}\xspace}
% \definecolor{purple}{rgb}{0.8,0.0,0.8}
% \def \bta {\mathbf{\bx}}
% \def \bu {\mathbf{u}}
% \def \bbS {\mathbb{S}}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argLexiMin}{arg\,lexi-min}

% \newcommand{\sz}[1]{\textcolor{blue}{[\textbf{sz:} #1]}}
% \newcommand{\sk}[1]{{\color{blue}{#1}}}
% \newcommand{\yr}[1]{\textcolor{purple}{[\textbf{yr:} #1]}}
% \newcommand{\qw}[1]{\textcolor{red}{[\textbf{QW:} #1]}}
% \newcommand{\todo}[1]{\textcolor{red}{[\textbf{TODO:} #1]}}

%--------Environments----------
\newtheorem{thm}{Theorem}%[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{exmp}{Example}
\newtheorem{rem}{Remark}
\newtheorem{assumption}[thm]{Assumption}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

